TRANSAX: A Blockchain-based Decentralized Forward-Trading Energy Exchange for Transactive Microgrids

Power grids are undergoing major changes due to rapid growth in renewable energy and improvements in battery technology. Prompted by the increasing complexity of power systems, decentralized IoT solutions are emerging, which arrange local communities into transactive microgrids. The core functionality of these solutions is to provide mechanisms for matching producers with consumers while ensuring system safety. However, there are multiple challenges that these solutions still face: privacy, trust, and resilience. The privacy challenge arises because the time series of production and consumption data for each participant is sensitive and may be used to infer personal information. Trust is an issue because a producer or consumer can renege on the promised energy transfer. Providing resilience is challenging due to the possibility of failures in the infrastructure that is required to support these market based solutions. In this paper, we develop a rigorous solution for transactive microgrids that addresses all three challenges by providing an innovative combination of MILP solvers, smart contracts, and publish-subscribe middleware within a framework of a novel distributed application platform, called Resilient Information Architecture Platform for Smart Grid. Towards this purpose, we describe the key architectural concepts, including fault tolerance, and show the trade-off between market efficiency and resource requirements.

==> feeder.tex <==
     \begin{figure}[t]
 \centering
\resizebox{0.45\textwidth}{!}{%
 \begin{tikzpicture}[rotate=270,font=\tiny,
   oc/.style={fill=black,rectangle,minimum size=0.01cm,font=\tiny},
     feeder/.style={fill=brown,rectangle,minimum size=0.005cm,font=\tiny},
   Producer/.style={fill=green,circle,minimum size=0.01cm},
     Consumer/.style={fill=red,circle,minimum size=0.01cm},
   Connection/.style={<->, >=stealth, shorten <=0.05cm, shorten >=0.05cm}]
 \draw node[oc] (oc1) at (-5,0){};
 \draw node[oc] (oc2) at (-4,0){};
 \draw node[oc] (oc3) at (-3,0){};
 \draw node[oc] (oc4)  at (-2,0){};
 \draw node[oc](oc5)  at (-1,0){};
 \draw node[oc] (oc6)  at (0,0){};
 \draw node[oc] (oc7) at (1,0){};
 \draw node[oc] (oc8)  at (2,0){};
 \draw node[oc] (oc9) at (3,0){};
 \draw node[oc] (oc10) at (4,0){};
 \draw node[oc] (oc11) at (5,0){};

 \draw node[feeder] (feeder1) at (-5,-1){};
 \draw node[feeder] (feeder2) at (-4,-1){};
 \draw node[feeder] (feeder3) at (-3,-1){};
 \draw node[feeder] (feeder4)  at (-2,-1){};
 \draw node[feeder](feeder5)  at (-1,-1){};
 \draw node[feeder] (feeder6)  at (0,-1){};
 \draw node[feeder] (feeder7) at (1,-1){};
 \draw node[feeder] (feeder8)  at (2,-1){};
 \draw node[feeder] (feeder9) at (3,-1){};
 \draw node[feeder] (feeder10) at (4,-1){};
 \draw node[feeder] (feeder11) at (5,-1){};

 \draw [Connection] (feeder1) to (feeder2);
 \draw [Connection] (feeder2) to (feeder3);
 \draw [Connection] (feeder3) to (feeder4);
 \draw [Connection] (feeder4) to (feeder5);
 \draw [Connection] (feeder5) to (feeder6);
 \draw [Connection] (feeder6) to (feeder7);
 \draw [Connection] (feeder7) to (feeder8);
 \draw [Connection] (feeder8) to (feeder9);
 \draw [Connection] (feeder9) to (feeder10);
 \draw [Connection] (feeder10) to (feeder11);

\draw [Connection] (feeder1) to (oc1);
\draw [Connection] (feeder2) to (oc2);
\draw [Connection] (feeder3) to (oc3);
\draw [Connection] (feeder4) to (oc4);
\draw [Connection] (feeder5) to (oc5);
\draw [Connection] (feeder6) to (oc6);
\draw [Connection] (feeder7) to (oc7);
\draw [Connection] (feeder8) to (oc8);
\draw [Connection] (feeder9) to (oc9);
\draw [Connection] (feeder10) to (oc10);
\draw [Connection] (feeder11) to (oc11);


 \foreach \pos in {1,2} {
   \node [Producer] (p10\pos)at (-5,\pos) {};
 }

 \foreach \pos in {3,4,5,6,7,8,9} {
   \node [Consumer] (c10\pos)at (-5,\pos) {};
 }

 \foreach \pos in {1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17} {
   \node [Consumer] (c20\pos)at (-4,\pos) {};
 }

 \foreach \pos in {1,2,3,4,5} {
   \node [Consumer] (c30\pos)at (-3,\pos) {};
 }


 \foreach \pos in {1,2,3,4,5,6,7,8,9,10,11,12,13} {
   \node [Consumer] (c40\pos)at (-2,\pos) {};
 }


 \foreach \pos in {1,2,3,4,5,6,7,8} {
   \node [Consumer] (c50\pos)at (-1,\pos) {};
 }


 \foreach \pos in {1} {
   \node [Consumer] (c60\pos)at (0,\pos) {};
 }


 \foreach \pos in {1} {
   \node [Producer] (p70\pos)at (1,\pos) {};
 }


 \foreach \pos in {2,3,4,5,6,7,8,9,10,11} {
   \node [Consumer] (c70\pos)at (1,\pos) {};
 }


 \foreach \pos in {17} {
   \node [Producer] (p80\pos)at (2,\pos) {};
 }

 \foreach \pos in {1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16} {
   \node [Consumer] (c80\pos)at (2,\pos) {};
 }

 \foreach \pos in {1,2,3,4,5} {
   \node [Consumer] (c90\pos)at (3,\pos) {};
 }

 \foreach \pos in {11} {
   \node [Producer] (p100\pos)at (4,\pos) {};
 }

 \foreach \pos in {1,2,3,4,5,6,7,8,9,10,12,13} {
   \node [Consumer] (c100\pos)at (4,\pos) {};
 }

 \foreach \pos in {1,2,3,4,5} {
   \node [Consumer] (c110\pos)at (5,\pos) {};
 }


 \draw [Connection] (oc1) to (p101);
 \draw [Connection] (p101) to (p102);
 \draw [Connection] (p102) to (c103);
 \draw [Connection] (c103) to (c104);
 \draw [Connection] (c104) to (c105);
 \draw [Connection] (c105) to (c106);
 \draw [Connection] (c106) to (c107);
 \draw [Connection] (c107) to (c108);
 \draw [Connection] (c108) to (c109);
 
\draw [Connection] (oc2) to (c201);
\draw [Connection] (c201) to (c202);
\draw [Connection] (c202) to (c203);
\draw [Connection] (c203) to (c204);
\draw [Connection] (c204) to (c205);
\draw [Connection] (c205) to (c206);
\draw [Connection] (c206) to (c207);
\draw [Connection] (c207) to (c208);
\draw [Connection] (c208) to (c209);
\draw [Connection] (c209) to (c2010);
\draw [Connection] (c2010) to (c2011);
\draw [Connection] (c2011) to (c2012);
\draw [Connection] (c2012) to (c2013);
\draw [Connection] (c2013) to (c2014);
\draw [Connection] (c2014) to (c2015);
\draw [Connection] (c2015) to (c2016);
\draw [Connection] (c2016) to (c2017);

\draw [Connection] (oc3) to (c301);
\draw [Connection] (c301) to (c302);
\draw [Connection] (c302) to (c303);
\draw [Connection] (c303) to (c304);
\draw [Connection] (c304) to (c305);

\draw [Connection] (oc4) to (c401);
\draw [Connection] (c401) to (c402);
\draw [Connection] (c402) to (c403);
\draw [Connection] (c403) to (c404);
\draw [Connection] (c404) to (c405);
\draw [Connection] (c405) to (c406);
\draw [Connection] (c406) to (c407);
\draw [Connection] (c407) to (c408);
\draw [Connection] (c408) to (c409);
\draw [Connection] (c409) to (c4010);
\draw [Connection] (c4010) to (c4011);
\draw [Connection] (c4011) to (c4012);
\draw [Connection] (c4012) to (c4013);

\draw [Connection] (oc5) to (c501);
\draw [Connection] (c501) to (c502);
\draw [Connection] (c502) to (c503);
\draw [Connection] (c503) to (c504);
\draw [Connection] (c504) to (c505);
\draw [Connection] (c505) to (c506);
\draw [Connection] (c506) to (c507);
\draw [Connection] (c507) to (c508);

\draw [Connection] (oc6) to (c601);

\draw [Connection] (oc7) to (p701);
\draw [Connection] (p701) to (c702);
\draw [Connection] (c702) to (c703);
\draw [Connection] (c703) to (c704);
\draw [Connection] (c704) to (c705);
\draw [Connection] (c705) to (c706);
\draw [Connection] (c706) to (c707);
\draw [Connection] (c707) to (c708);
\draw [Connection] (c708) to (c709);
\draw [Connection] (c709) to (c7010);
\draw [Connection] (c7010) to (c7011);

\draw [Connection] (oc8) to (c801);
\draw [Connection] (c801) to (c802);
\draw [Connection] (c802) to (c803);
\draw [Connection] (c803) to (c804);
\draw [Connection] (c804) to (c805);
\draw [Connection] (c805) to (c806);
\draw [Connection] (c806) to (c807);
\draw [Connection] (c807) to (c808);
\draw [Connection] (c808) to (c809);
\draw [Connection] (c809) to (c8010);
\draw [Connection] (c8010) to (c8011);
\draw [Connection] (c8011) to (c8012);
\draw [Connection] (c8012) to (c8013);
\draw [Connection] (c8013) to (c8014);
\draw [Connection] (c8014) to (c8015);
\draw [Connection] (c8015) to (c8016);
\draw [Connection] (c8016) to (p8017);

\draw [Connection] (oc9) to (c901);
\draw [Connection] (c901) to (c902);
\draw [Connection] (c902) to (c903);
\draw [Connection] (c903) to (c904);
\draw [Connection] (c904) to (c905);

\draw [Connection] (oc10) to (c1001);
\draw [Connection] (c1001) to (c1002);
\draw [Connection] (c1002) to (c1003);
\draw [Connection] (c1003) to (c1004);
\draw [Connection] (c1004) to (c1005);
\draw [Connection] (c1005) to (c1006);
\draw [Connection] (c1006) to (c1007);
\draw [Connection] (c1007) to (c1008);
\draw [Connection] (c1008) to (c1009);
\draw [Connection] (c1009) to (c10010);
\draw [Connection] (c10010) to (p10011);
\draw [Connection] (p10011) to (c10012);
\draw [Connection] (c10012) to (c10013);


\draw [Connection] (oc11) to (c1101);
\draw [Connection] (c1101) to (c1102);
\draw [Connection] (c1102) to (c1103);
\draw [Connection] (c1103) to (c1104);

 \end{tikzpicture}
 }
 \caption{Feeder diagram. Brown nodes are feeder junctions, numbered 1 to 11 from top to bottom.  Black nodes are the overcurrent relays, which ensure that the total power flowing in and out of the feeder is below 20 kW. The green nodes are the junction points for the producers ($5$), and the red nodes are junction points for the consumers ($97$). There are $102$ prosumers in total.}
 \label{fig:feeder}
 \end{figure}
